One Step Closer: Creating the Future to Boost Monocular Semantic Scene Completion

In recent years, visual 3D Semantic Scene Completion (SSC) has emerged as a critical perception task for autonomous driving due to its ability to infer complete 3D scene layouts and semantics from single 2D images. However, in real-world traffic scenarios, a significant portion of the scene remains occluded or outside the camera's field of view -- a fundamental challenge that existing monocular SSC methods fail to address adequately. To overcome these limitations, we propose Creating the Future SSC (CF-SSC), a novel temporal SSC framework that leverages pseudo-future frame prediction to expand the model's effective perceptual range. Our approach combines poses and depths to establish accurate 3D correspondences, enabling geometrically-consistent fusion of past, present, and predicted future frames in 3D space. Unlike conventional methods that rely on simple feature stacking, our 3D-aware architecture achieves more robust scene completion by explicitly modeling spatial-temporal relationships. Comprehensive experiments on SemanticKITTI and SSCBench-KITTI-360 benchmarks demonstrate state-of-the-art performance, validating the effectiveness of our approach, highlighting our method's ability to improve occlusion reasoning and 3D scene completion accuracy.

==> README <==

January 11, 2007


IEEEtran.bst is the official BibTeX style for authors of the Institute of
Electrical and Electronics Engineers (IEEE) Transactions journals and
conferences.

It also may have applications for other academic work such as theses and
technical reports. The alphanumeric and natbib variants extend the
applicability of the IEEEtran bibstyle family to the natural sciences
and beyond.

The IEEEtran bibstyle is a very comprehensive BibTeX style which provides
many features beyond the standard BibTeX styles, including full support
for references of online documents, patents, periodicals and standards.
See the provided user manual for detailed usage information.

The latest version of the IEEEtran BibTeX style can be found at CTAN:

http://www.ctan.org/tex-archive/macros/latex/contrib/IEEEtran/bibtex/

as well as within IEEE's site:

http://www.ieee.org/

Note that the packages at IEEE's site do not contain the natbib and
alphanumeric variants (e.g., IEEEtranN.bst, etc.) as these are not used
for IEEE related work. These files can be obtained on CTAN.

For helpful tips, answers to frequently asked questions and other support,
visit the IEEEtran home page at my website:

http://www.michaelshell.org/tex/ieeetran/


Enjoy!

Michael Shell
http://www.michaelshell.org/

*******
Version 1.12 (2007/01/11) changes:

 1. Fixed bug with unwanted comma before "et al." when an entry contained
    more than two author names. Thanks to Pallav Gupta for reporting this.

 2. Fixed bug with anomalous closing quote in tech reports that have a
    type, but without a number or address. Thanks to Mehrdad Mirreza for
    reporting this.

 3. Use braces in \providecommand in begin.bib to better support
    latex2html. TeX style length assignments OK with recent versions
    of latex2html - 1.71 (2002/2/1) or later is strongly recommended.
    Use of the language field still causes trouble with latex2html.
    Thanks to Federico Beffa for reporting this.

 4. Added IEEEtran.bst ID and version comment string to .bbl output.

 5. Provide a \BIBdecl hook that allows the user to execute commands
    just prior to the first entry.

 6. Use default urlstyle (is using url.sty) of "same" rather than rm to
    better work with a wider variety of bibliography styles.

 7. Changed month abbreviations from Sept., July and June to Sep., Jul.,
    and Jun., respectively, as IEEE now does. Thanks to Moritz Borgmann
    for reporting this.

 8. Control entry types should not be considered when calculating longest
    label width.

 9. Added alias www for electronic/online.

10. Updated full and abbreviated journal name string definitions in
    IEEEfull.bib and IEEEabrv.bib.

11. New IEEEtranSA.bst, IEEEtranN.bst, and IEEEtranSN.bst variants for
    alphanumeric citation tags and natbib compatibility.


********************************** Files **********************************

README                 - This file.

IEEEtran_bst_HOWTO.pdf - The user manual.

IEEEtran.bst           - The standard IEEEtran BibTeX style file. For use
                         with IEEE work.

IEEEtranS.bst          - A version of IEEEtran.bst that sorts the entries.
                         Some IEEE conferences/publications may use/allow
                         sorted bibliographies.

IEEEexample.bib        - An example BibTeX database that contains the
                         references shown in the user manual.

IEEEabrv.bib           - String definitions for the abbreviated names of
                         IEEE journals. (For use with IEEE work.)
                         
IEEEfull.bib           - String definitions for the full names of IEEE
                         journals. (Do not use for IEEE work.)


Carried on CTAN only, for non-IEEE related work:

IEEEtranSA.bst         - Like IEEEtranS.bst, but with alphanumeric citation
                         tags like alpha.bst. Not for normal IEEE use.

EEEtranN.bst          - Like IEEEtran.bst, but based on plainnat.bst and
                         is compatible with Patrick W. Daly's natbib
                         package. Not for normal IEEE use.

IEEEtranSN.bst         - Sorting version of IEEEtranN.bst. Not for normal
                         IEEE use

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran_bst_HOWTO.pdf, IEEEtran.bst, IEEEtranS.bst,
                   IEEEtranSA.bst, IEEEtranN.bst, IEEEtranSN.bst,
                   IEEEexample.bib, IEEEabrv.bib, IEEEfull.bib
                   
***************************************************************************


==> secs/rebuttal.tex <==
\begin{figure*}[htbp]
  \centering
  \includegraphics[width=0.9\linewidth]{figs/fig2.jpg}
   %\includegraphics[width=0.8\linewidth]{egfigure.eps}
   \caption{Overall framework of our proposed CF-SSC, which takes images and poses of past frames and the current frame as input, predicts images, depth, and relative poses of future frames, and integrates all temporal information for SSC.}
   \label{fig:re}
\end{figure*}
\section{Rebuttal}
Due to space limitations and the complexity of the overall framework, we were unable to elaborate on certain implementation details in the paper. Therefore, we provide further clarifications in the rebuttal.
\subsection{Regarding Technical Details and Reproducibility}
Regarding reproducibility, we will release our code on "https://github.com/luang321/CF-OCC" after the final decision of the paper, along with the pretrained model and the corresponding testing results.

As mentioned in the paper, and shown in Fig.\ref{fig:re}, our framework includes a SpatialTemporal SSC module for fusing spatiotemporal information to perform SSC prediction, a FuturePoseNet for predicting the poses of future frames, and a FutureSynthNet for generating future frame images and depth maps. We first train SpatialTemperol SSC and FuturePoseNet, and then train FutureSynthNet based on the image encoder of SpatialTemperol SSC. 

In FuturePoseNet, following the design of Symphonies\cite{jiang2024symphonize}, our image encoder adopts the ResNet-50\cite{he2016deep} backbone from the pretrained MaskDINO\cite{li2023mask} model(See the implementation details section of the paper.), while the pose encoder is implemented using a 3-layer MLP network. In FutureSynthNet, the 2D U-Net performs downsampling using three convolution-BatchNorm-ReLU blocks, and applies the same module for upsampling by replacing the convolution layers with transposed convolutions.

For Spatial-Temporal SSC, following the design of FuturePoseNet, we also adopt the pretrained ResNet-50\cite{he2016deep} from MaskDINO\cite{li2023mask} as the image encoder. The 3D U-Net follows the implementation used in \cite{cao2022monoscene} and \cite{roldao2020lmscnet}(See the implementation details section of the paper.), performing two stages of downsampling and upsampling on the 3D features. To reduce the number of parameters, each $3\times3\times3$ convolution in the downsampling and upsampling blocks is decomposed into three sequential $3\times1\times1$ convolutions along different dimensions.

As for the depth network, we adopt the off-the-shelf method from \cite{li2023voxformer}, which is also a common practice in monocular SSC tasks and has been used by methods such as \cite{jiang2024symphonize,zheng2024monoocc,wang2024h2gformer,wang2024not,yao2023depthssc}.

All sampling operations are performed using bilinear interpolation. Other implementation details are provided in the paper.


We train our model using 4 NVIDIA RTX 4090 GPUs. Following previous methods\cite{cao2022monoscene}, we set the batch size to 4 and employ the AdamW\cite{loshchilov2017decoupled} optimizer for 30 epochs. The initial learning rate is set to 1e-4 with weight decay of 1e-4, and the learning rate is reduced by a factor of 0.1 at the 20th and 25th epochs.Additionally,  we use a frame interval of 5 frames between consecutive inputs(See the implementation details section of the paper.).
\begin{figure*}[htbp]
  \centering
  \includegraphics[width=0.9\linewidth]{figs/occ.jpg}
   %\includegraphics[width=0.8\linewidth]{egfigure.eps}
   \caption{Visualization of occlusion.}
   \label{fig:occ}
\end{figure*}
\subsection{Regarding Losses}
Since loss functions such as L1 and cross-entropy (CE) are common sense, we did not elaborate on them in the paper.

As mentioned in the paper, we use the MSE loss to supervise the pose prediction, which is a common practice in visual odometry tasks. Therefore, the loss between the predicted pose $P_{t+1}^p$ and the ground-truth pose $P_{t+1}$ matrices can be formulated as:
\begin{equation}
L_{mse}^{p} = \frac{1}{N} \sum_{i=1}^{N} (P_{t+1}^p - P_{t+1})^2
\end{equation}

As mentioned in the paper, we apply L1 and SSIM losses at the image level for the pseudo images $I_{t+1}^p$ predicted by FutureSynthNet. These pseudo images are then passed through the pretrained image encoder from Spatial-Temporal SSC to obtain feature representations, where we further apply an L1 loss at the feature level. Additionally, we apply an L1 loss to supervise the predicted depth maps $D_{t+1}^p$. The corresponding losses can be formulated as follows:

\begin{equation}
L_{l1}^{img} = \frac{1}{HW} \sum_{x=1}^{H} \sum_{y=1}^{W}  \left|I_{t+1}^p-I_{t+1} \right|
\end{equation}
\begin{equation}
L_{l1}^{feat} = \frac{1}{HW} \sum_{x=1}^{H} \sum_{y=1}^{W}  \left|enc(I_{t+1}^p)-enc(I_{t+1}) \right|
\end{equation}

\begin{equation}
L_{l1}^{d} = \frac{1}{HW} \sum_{x=1}^{H} \sum_{y=1}^{W}  \left|D_{t+1}^p-D_{t+1} \right|
\end{equation}
and 
\begin{equation}
L_{ssim}^{img} = 1 - ssim(I_{t+1}^p,I_{t+1})
\end{equation}
where $enc()$ denotes the result obtained by forwarding through the image encoder.

For SpatioTemporal SSC specifically, as mentioned in the paper, following \cite{cao2022monoscene}, we employ Scene-Class Affinity Loss $L_{scal}$ with dual supervision on both geometric and semantic aspects, combined with cross-entropy loss weighted by class frequencies. The complete loss function is formulated as:
\begin{equation}
L_{ssc} = L_{scal}^{geo} + L_{scal}^{sem} +L_{ce}
\end{equation}

For $L_{scal}$, suppose the predicted SSC probability distribution is denoted as $\hat{p_{i,c}}$, $L_{scal}$ optimize the class-wise derivable (P)precision,(R)ecall and (S)pecificity, where $P_c$ and  $R_c$ measure the performance of similar class $c$ voxels, and $S_c$ measures the performance of dissimilar voxels( not of class $c$). Considering $p_i$ the fround truth class of voxel $i$:

\begin{align}
P_c(\hat{p}, p) &= \log \frac{\sum_i \hat{p}_{i,c} \, \mathbb{I}[p_i = c]}{\sum_i \hat{p}_{i,c}}, \\
R_c(\hat{p}, p) &= \log \frac{\sum_i \hat{p}_{i,c} \, \mathbb{I}[p_i = c]}{\sum_i \mathbb{I}[p_i = c]}, \\
S_c(\hat{p}, p) &= \log \frac{\sum_i (1 - \hat{p}_{i,c}) \, (1 - \mathbb{I}[p_i = c])}{\sum_i (1 - \mathbb{I}[p_i = c])},
\end{align}

\begin{equation}
    \mathcal{L}_{\text{scal}}(\hat{p}, p) = -\frac{1}{C} \sum_{c=1}^{C} \left( P_c(\hat{p}, p) + R_c(\hat{p}, p) + S_c(\hat{p}, p) \right)
\end{equation}
$L_{scal}^{sem}$ is computed over all categories and averaged, while $L_{scal}^{geo}$  is computed only over voxels that are valid (i.e., non-empty) in the scene.
\begin{equation}
\mathcal{L}_{ce} = - \left[ p \log(\hat{p}) + (1 - p) \log(1 - \hat{p}) \right]
\end{equation}
The weight for the $L_{mse}^{p}$ loss is set to 0.1, and the weights for all other losses are set to 1.

\subsection{Regarding Occlusion}
As shown in the Fig.\ref{fig:occ}, to prevent the generation of erroneous information, we constrain the generated images at the level of primary features, mainly using the L1 loss. As a result, the generated images are not sharp. When dealing with mildly occluded regions, our network can reconstruct them relatively well.As shown in the last row of the Fig.\ref{fig:occ} However, for severely occluded areas, our method fails to handle them effectively.

